Joint System-Wise Optimization for Pipeline Goal-Oriented Dialog System

Recent work (Takanobu et al., 2020) proposed the system-wise evaluation on dialog systems and found that improvement on individual components (e.g., NLU, policy) in prior work may not necessarily bring benefit to pipeline systems in system-wise evaluation. To improve the system-wise performance, in this paper, we propose new joint system-wise optimization techniques for the pipeline dialog system. First, we propose a new data augmentation approach which automates the labeling process for NLU training. Second, we propose a novel stochastic policy parameterization with Poisson distribution that enables better exploration and offers a principled way to compute policy gradient. Third, we propose a reward bonus to help policy explore successful dialogs. Our approaches outperform the competitive pipeline systems from Takanobu et al. (2020) by big margins of 12% success rate in automatic system-wise evaluation and of 16% success rate in human evaluation on the standard multi-domain benchmark dataset MultiWOZ 2.1, and also outperform the recent state-of-the-art end-to-end trained model from DSTC9.

==> preliminaries.tex <==
\section{Preliminaries on Pipeline Dialogue System}

%\subsection{Dialogue System Architectures}
%pipeline system; joint; end-to-end
%\subsection{Pipeline Dialogue System}
%NLU, DST, Policy, NLG
%NLU: input, output, training loss
%Policy: input, output, PPO
%\jing{Again I think having a figure that shows these high level components, as well as adding details of each component: intent/slot for NLU, etc, would make reviewers easy to follow the text, make the paper self-contained. Also, can we replace BERTNLU by BERT-NLU? in the system paper they just used BERT. I think maybe you want to emphasize BERT used for NLU? so BERT-NLU is more appropriate.}


%\paragraph{\textit{Natural Language Understanding}}
\subsection{Natural Language Understanding (NLU)}
%\tnote{some citations. (There are a few that I commented out in the intro)} 

%\tnote{use a running exmple for this entire section, so that you can ground everythign with a concerte example. Perhaps use the same example in the figure if appilcable}

%\jing{this paragraph is not needed. Try without it?}
%The NLU component~\cite{devlin2018bert,radford2018improving,zheng2020out} maps the utterances to structured information that represents the intent and values of the utterances. A popular schema is the dialog act~\cite{stolcke2000dialogue}, which consists of intent and slot-values. The intent type is a high-level representation of an utterance, such as \textit{Request} and \textit{Inform}. Slot-value pairs are the task-specific semantic elements that are mentioned in an utterance. Take Figure~\ref{fig:pipeline} as an example. The system NLU takes the users' utterance ``I want to find a Chinese restaurant'' as input, and then detect the intents (``Inform'') and slot-values (``\{Food: Chinese\}'') to form a dialog act (``Inform-Restaurant-Food-Chinese'').

%As the example suggested, the 
The task of NLU~\cite{devlin2018bert,radford2018improving,zheng2020out} is typically decomposed into two sub-tasks: intent detection and slot-value extraction. 
%The former is normally formulated as an intent classification task with the utterances as inputs, and the latter is often viewed as a problem of labeling each token in the sequence by its corresponding slot (or labeling by ``no slot'').
We will use $d$ to denote the dialog act, and $u$ to denote the utterance. The NLU components $f_{\omega}$ maps an utterance to the corresponding dialog act $d$. 
Another important notion is the delexicalized dialog act, denoted by $\bar{d}$, which will be combined with the slot value from the database to result in a full dialog act.
%which substitutes the slot in the dialog act to a number (e.g., ``Inform-Restaurant-Food-1'') --- the number will be refilled by a value queried from database for lexiclization.
%\tnote{say give a informal def, an example, and also say it's one of out 209 choices}


We describe the intent classification problem below in more detail as they are relevant in our algorithm. Let us denote the function of slot classification as $f^{slot}$ which maps the utterance $u$ of $k$ tokens to a sequence of $k$ slot IDs, one for each tokens. (Each token can be classified into one of the slots, or no slot). Let $f^{intent}$ denote function of intent detection, which maps an utterance $u$ to one of the possible intents. We use pre-trained BERT~\cite{devlin2018bert} to get token/sentence embedding and add two linear classifiers for the tasks. We use cross entropy loss to train both the slot classification and the intent detection tasks (in the former case, we use the sum of the cross-entropy losses over all tokens). 
Let $\omega$ denote all the parameters and let 
%Denoting the slot label as $y_{slot} \in \cR^n$ and the intent label as $y_{intent} \in \cR^m$, we train the NLU by minimizing the following cross entropy losses:
%We can get slot label $y_{slot}$ and intent label $y_{intent}$ from dialog act, and enforce consistency by minimizing the following losses:
%\small
$\cL_{slot}(\omega)$ and $\cL_{intent}(\omega)$ denote the two losses and the final loss function is the their sum 
\begin{equation} \label{eq:nluloss}
\cL_{slot}(\omega) + \cL_{intent}(\omega) 
\end{equation}
% {
% \begin{equation}\label{eq:slot}
%     \cL_{slot}(u) = - \log \left( \frac{\exp(f_{\omega}^{slot}(u)_{y_{slot}})}{\sum_j \exp(f_{\omega}^{slot}(u)_j)} \right) ,
% \end{equation}
% \begin{equation}\label{eq:intent}
% \begin{aligned}
%     \cL_{intent}(u) &= y_{intent} \log \sigma(f_{\omega}^{intent}(u)) + \\ &  (1-y_{intent}) \log (1-\sigma(f_{\omega}^{intent}(u))).
% \end{aligned}
% \end{equation}
%\tnote{just say learn by SGD with learning rate $\alpha$. No need to say $\alpha$ even if you don't need to use that symbol later.}

% \begin{equation}\label{eq:nluloss}
%     \omega \leftarrow \omega - \alpha \nabla_{\omega} (\cL_{slot}(u) + \cL_{intent}(u)) ,
% \end{equation}
% }
% where $\alpha$ is the learning rate of the parameter of NLU.

%\paragraph{\textit{Dialog State Tracking}}
\subsection{Dialog State Tracking (DST)}
%The dialog state tracker (DST) estimates the user's goal in each time step by taking the entire dialog context as input. The dialog state at time $t$ can be regarded as an abstracted representation of the previous turns until t. Most existing works adopted belief state for dialog state representation

A DST infers the belief state (or user goal) from dialog history. It receives the intents and slot-values from NLU and outputs a belief state, which encodes the extracted information as a compact set of dialog state that contains a set of informable slots and their corresponding values (user constraints), and a set of requested slots. The belief state is often used to query a task-specific database (DB) to obtain the DB state, such as the number of entities that match the user goal.

%A dialog state tracker encodes the extracted information as a compact set of dialog state that contains a set of informable slots and their corresponding values (user constraints), and a set of requested slots

%The dialog state tracker (DST) estimates the user's goal in each time step by taking the entire dialog context as input. The dialog state at time t can be regarded as an abstracted representation of the previous turns until t. Most existing works adopted belief state for dialog state representation, in which the state is composed of several probability distributions over the value vocabulary of each slot. Therefore, this problem can be formulated as a multi-task classification task:
%\begin{equation}
%    p_i(d_{i,t} | u_1, u_2, ..., u_t),
%\end{equation}
%\tnote{this is quite confusing. I thougth the input to the DST is intent and slot values instead of utterances, and I thought it's deterministic. We should stress the input/ouput interfaces and deterministic nature.}
%\tnote{Also explain the query of database, etc.}
%\tnote{the general guideline for this section and NLG section is that you want to emphasize more about the interfaces (what are input and outputs, what are the form of inputs and outputs), but you don't have to talk much about details on the exact implmentation. E.g., you should want to say clearly what's the dimensionality of output of the DST. } \zichuan{add more description about the interfaces}
%where for each specific slot $i$, there is a tracker $p_i$. $u_t$ represents the utterance in turn $t$. The class of slot $i$ in the $t$-th turn is $d_{i,t}$.

%\paragraph{\textit{Dialog Policy}}
\subsection{Dialog Policy}
%\tnote{specify the input and output space. E.g., what is the input to the policy (what dimensionality), and what's the form of the outputs.} \zichuan{specified the input and output space and their form}
Conditioned on the dialog state, the dialog policy generates the next system action. Since the dialog acts in a session are generated sequentially, it is often formulated as a Markov Decision Process (MDP), which can be addressed by Reinforcement Learning (RL). The dialog state consists of (1) belief state; (2) DB state; (3) user actions at current turn; (4) system actions at the last turn. The dialog state is then vectorized as a binary vector which serves as the input of policy. Given the input, the policy then outputs a distribution over all candidate delexicalized dialog acts and sample actions from that distribution.
Denoting the state space as $\cS$, the action space as $\cA$, the policy learns to map the state to action: $\pi_{\theta}: \cS \rightarrow \cA$, where $\theta$ is the parameters of policy. At the $t$-th turn, the policy faces a state $s_t\in \cS$, takes an action $a_t \in \cA$ and receive a reward $r_t \in \cR$. In this paper, we use proximal policy optimization (PPO)~\cite{schulman2017proximal} and train our policy by maximizing:
\begin{equation} \label{eq:ppo}
\scriptsize{
    \mathrm{min} \left( \frac{\pi_{\theta}(a_t|s_t)}{\pi_{old}(a_t|s_t)} A_t, \mathrm{clip} \left(\frac{\pi_{\theta}(a_t|s_t)}{\pi_{old}(a_t|s_t)}, 1-\epsilon, 1+\epsilon \right) A_t  \right),
}
\end{equation}
where $\epsilon$ is a hyper-parameter of PPO and $A_t$ is the advantage function. Following common practice~\cite{takanobu2020your}, we use a sparse reward function --- we give a positive reward $2L$ for a success dialog and a negative reward $-L$ for a failure one, where $L$ represents the number of dialog turns. we denote this reward function as $r_{origin}$.

%\zichuan{describe commonly used policy network architecture}
%\zichuan{imitation learning loss}

%\paragraph{\textit{Natural Language Generation}}
\subsection{Natural Language Generation (NLG)}
Given the dialog act generated by the dialog policy, the NLG component maps the act to a natural language utterance, which is often modeled as a conditioned language generation task~\cite{wen2015semantically}. To improve user experience, the generated utterance should (1) fully convey the semantics of a dialog act for task-completion, and (2) be natural, specific, and informative, analogous to human language. In this paper, we apply a retrieval-based NLG implemented in Convlab-2~\cite{zhu2020convlab}.

%define notation
%component-wise training for a pipeline system

% Jing: remove these two sections to save space
%\subsection{Pipeline System with Modular Training}
%In the existing pipeline systems, all these modules are component-wise trained with their own fine-grained supervision signals and overlook the relationship to other modules. Therefore, when they are assembled together, one module may be sensitive to the errors induced by its upstream models, and thus the system-wise evaluation performance is not always consistent with the component-wise evaluation performance.

%\subsection{System-wise Evaluation}
%Figure~\ref{fig:pipeline} shows the entire workflow in a pipeline dialogue system. The system consists of NLU, DST, Policy and NLG, which takes in user utterances outputs system utterances. The user consists of an NLU, an NLG and an agenda-based user simulator~\cite{schatzmann2007agenda}. For fair comparison, we follow the state-of-the-art configuration rule-based system~\cite{takanobu2020your}, which uses BERT-NLU, rule-based DST, rule-based policy and retrieval-based NLG --- BERT-NLU is a fine-tuned BERT model~\cite{devlin2018bert} for NLU; rule-based DST is implemented in Convlab-2~\cite{zhu2020convlab}; retrieval-based NLG samples a sentence randomly from the corpus using dialog acts~\cite{takanobu2020your}.

% \subsection{System-wise RL Training}
% To overcome the issue above, an intuitive way is to perform system-wise RL training, which views other modules (NLU, DST, NLG) as parts of the environment and trains the policy to adapt to the entire dialogue system.


% However, we observe that system-wise RL training does not work well because of domain shift and compounding errors.




%system-wise training for a pipeline system
